Resource Allocation in Wireless Networks with Energy Constraints

This dissertation focuses on the development of novel scheduling and resource allocation schemes, which take into account and regulate the energy constraints imposed by the levels of harvested energy. To this direction, first, the optimal energy, time, and bandwidth allocation problem for the downlink of energy harvesting base stations (EHBSs) is investigated, with the main focus being on autonomous EHBSs. The presented analysis considers the impact of the energy constraint on users' preferences and the BS's revenue. In order to model the competitive nature of the problem, game theory is used. The next two chapters focus on wireless powered networks (WPNs) and simultaneous wireless information and power transfer (SWIPT) using radio frequency (RF) technology. One of the main contributions of these chapters is the introduction of both uplink and downlink non-orthogonal multiple access (NOMA) for WPNs. Moreover, the individual data rates and fairness are improved, while the formulated problems are optimally and efficiently solved. It is shown that, compared to orthogonal multiple access, NOMA offers a considerable improvement in throughput, fairness, and energy efficiency. Rather than this, proportional fairness is maximized and uplink/downlink of WPNs are jointly optimized, in which cases, except for NOMA, time division multiple access (TDMA) is also investigated. Furthermore, the role of interference is considered, which has been recognized as one of the main reasons of the asymmetric overall degradation of the users' performance, due to different path-loss values, called from now on as cascaded near-far problem. Moreover, SWIPT is investigated and efficiently optimized in the context of multicarrier cooperative communication networks. Finally, simultaneous lightwave information and power transfer (SLIPT) is introduced, while novel and fundamental techniques are proposed.

==> 3.lists/nomenclature_copy.tex <==
\chapter{List of Symbols}\label{ch:nomenclature}


\begin{table}[!h]\renewcommand{\arraystretch}{1.2}
\begin{tabular}{m{3.5cm}l}
$\mathbb{R}^n$&$n$-dimensional space of real numbers\\
$\mathbb{Z}^n$&$n$-dimensional space of integer numbers / $n$-dimensional integer lattice\\
$\Lambda$&lattice\\
$\mathrm{det}(\cdot)$&matrix determinant\\
$\mathrm{Vol}(\cdot)$&volume\\
$Q_\Lambda(\mathbf{x})$&lattice quantizer\\
$[\cdot]\mod\Lambda$&modulo - lattice operation\\
$\mathcal{V}$&Voronoi cell\\
$N_0$&noise power spectral density\\
$\mathbb{E}[\cdot]$&expected value\\
$P_e$&probability of error\\
$\mathrm{Pr}(\cdot)$&probability\\
$|\cdot|$&absolute value / set cardinality\\
$||\cdot||$&vector norm\\
$\mathrm{diag}\{\ldots\}$&diagonal matrix\\
$\mathbb{A}^2$&hexagonal lattice in $\mathbb{R}^2$\\
$G_p$&Gray code penalty\\
$f_x(x)$&probability density function of $x$\\
$F_x(x)$&cumulative distribution function of $x$\\
$\Gamma(\cdot)$&Gamma function\\
$\Gamma(\cdot,\cdot)$&upper incomplete Gamma function\\
$\gamma(\cdot,\cdot)$&lower incomplete Gamma function\\
$\mathcal{F}_n$&parallelotope facet of dimension $n$\\
$\binom{a}{b}$&binomial coefficient\\
$_2F_1(\alpha,\beta;\gamma;z)$&Gauss Hypergeometric function\\
$G_{p,q}^{m,n}\left[x\left|\begin{array}{c}\alpha_1,\ldots,\alpha_p\\\beta_1,\ldots,\beta_q\end{array}\right.\right]$&Meijer's G-function\\
$\Re{\mathbf{x}}$&real part of complex vector $\mathbf{x}$\\
$\Im{\mathbf{x}}$&imaginary part of complex vector $\mathbf{x}$\\
$(\cdot)^*$&conjuate\\
$(\cdot)^T$&transpose\\
$(\cdot)^H$&conjugate transpose\\
$\mathbb{F}_p$&$p$-sized field\\
$\bigoplus$&sum over a field\\
$\log_2^+(\cdot)$&$\max(0,\log_2(\cdot))$\\
$\mathbf{I}_{L\times L}$&identity matrix of dimension $L\times L$\\
$J_n(x)$&$n$-th order Bessel function of the first kind\\
$I_n(x)$&$n$-th order modified Bessel function of the first kind\\
$_1F_1(a,b,x)$&Kummer confluent Hypergeometric function\\
\end{tabular}
\end{table}

\begin{table}[!h]\renewcommand{\arraystretch}{1.2}
\begin{tabular}{m{3.5cm}l}
$Q_M(a,b)$&Marcum Q-function\\
$Q_{M,N}(a,b)$&Nuttall Q-function\\
$\succeq$&preference relation\\
$\succ$&strict preference relation\\
$\sim$&indifference relation\\
$\pi^*$&core partition\\
$\mathrm{sgn}(\cdot)$&sign function\\

\end{tabular}
\end{table}


%%Use one of the two modified versions of \nomenclature{symbol}{description} command:
%%1.\nomenclaturesortright{TAG}{symbol}{description}, that sorts the items according to their DESCRIPTION
%%2.\nomenclaturesortline{TAG}{symbol}{description}, that sorts the items according to their #line in the EDITOR
%%Note: TAG is a letter that denotes a particular group within the Nomenclature. Here the following rules apply:
%%TAG = C -> \nomgroup = Complex Numbers
%%TAG = D -> \nomgroup = Distributions
%%TAG = F -> \nomgroup = Functions
%%TAG = H -> \nomgroup = Set Theory
%%TAG = M -> \nomgroup = Matrices \& Vector Spaces
%%TAG = O -> \nomgroup = Operators
%%TAG = R -> \nomgroup = Random Variables
%%TAG = S -> \nomgroup = Stochastic Processes
%%TAG = T -> \nomgroup = Transformations \& Mappings
%%TAG = Z -> \nomgroup = Other Notations
%%...(for each line you add, update the corresponding commands in the preamble.tex file)
%
%%Symbols and notations for arena chapter (testing)
%\ifarenachapterflag
%
%\nomenclaturesortright{Z}{$\bigotimes$}{This is a classical symbol}%
%\nomenclaturesortright{Z}{$\mathbf{\Omega}$}{Greek capital letter in bold}%
%\nomenclaturesortright{Z}{$\sgn$}{This is a new defined function}%
%
%\else\fi
%
%%Symbols and notations for chapter 1
%\ifchapteroneflag
%
%\nomenclaturesortright{C}{$\re{z}$, $\im{z}$}{Real and imaginary parts of complex number $z$}%
%
%\else\fi
%
%%Symbols and notations for chapter 2
%\ifchaptertwoflag
%
%\nomenclaturesortright{C}{$\abs{z}$, $\angle{z}$}{Amplitude ($\abs{z}=a$) and phase ($\angle{z}=\theta$) of complex $z=ae^{\jmath\theta}$}%
%\nomenclaturesortright{C}{$\jmath=\sqrt{-1}$}{Imaginary unit (not to be confused with the index $j$)}%
%
%\nomenclaturesortright{D}{$x\sim\mathcal{N}(\mu_x,\sigma_x^2)$}{Normal (or Gaussian) distribution, $x\in\mathds{R}$}%
%\nomenclaturesortright{D}{$\boldi{z}\sim\mathcal{CN}(\boldn{0}_{m},\mathrm{K}_{\boldi{z}})$}{Circularly-symmetric complex Gaussian distribution, $\boldi{z}\in\mathds{C}^{m}$}%
%\nomenclaturesortright{D}{$x\sim\mathcal{U}(a,b)$}{Uniform distribution, $x\in\text{[}a,b\text{]}$ ($a$ and/or $b$ may be excluded)}%
%\nomenclaturesortright{D}{$x\sim\mathrm{Gamma}(\mu_x,1)$}{Standard Gamma distribution, $x\in\mathds{R}^{+}$}%
%\nomenclaturesortright{D}{$x\sim\chi_{k,\lambda}^2$}{Noncentral chi-square distribution with $k$ degrees of freedom and noncentrality parameter $\lambda>0$, $x\in\mathds{R}_{0}^{+}$}%
%
%\nomenclaturesortright{F}{$\Pi\left(\frac{x-x_{0}}{x_{w}}\right)\equiv\rect\left(\frac{x-x_{0}}{x_{w}}\right)$}{Rectangular function centered at $x_{0}$ of width $x_{w}$}%
%\nomenclaturesortright{F}{$\sinc(x)=\frac{\sin{(\pi x)}}{\pi x}$}{Normalized sinc function}%
%\nomenclaturesortright{F}{$\binom{m}{n}=\frac{m"!}{n"!(m-n)"!}$}{Binomial coefficient for $m,n\in\mathds{N}_0$, $m\geq n$}%
%\nomenclaturesortright{F}{$(m)_n=\frac{(m+n-1)"!}{(m-1)"!}$}{Rising factorial (Pochhammer's symbol) for $m\in\mathds{N}$, $n\in\mathds{N}_0$}%
%\nomenclaturesortright{F}{$n"!=\prod_{k=1}^n k$}{Factorial of $n\in\mathds{N}$ ($\triangleq 1$ for $n=0$)}%
%\nomenclaturesortright{F}{$\Psi(a,c;x)$}{Confluent hypergeometric function of the second kind}%
%\nomenclaturesortright{F}{$L_n(x)$}{Laguerre polynomial of degree $n$}%
%\nomenclaturesortright{F}{$L_n^{\alpha}(x)=\sum_{r=0}^{n}(-1)^r\binom{n+\alpha}{n-r}\frac{x^r}{r"!}$}{Generalized Laguerre polynomial of degree $n$ and order $\alpha$ with $L_n^{0}(x)\triangleq L_n(x)$ being the Laguerre polynomial of degree $n$}%
%\nomenclaturesortright{F}{$I_N(x)$}{Modified Bessel function of the first kind of order $N$}%
%\nomenclaturesortright{F}{$\sgn(z)=\frac{z}{\abs{z}}$}{Signum function with $\sgn(z)=z/\abs{z}$ for $z\neq 0$; $=0$ for $z=0$}%
%\nomenclaturesortright{F}{$Q(\alpha,\beta)=\int_\beta^\infty xe^{-\frac{x^2+\alpha^2}{2}}I_0(\alpha x)dx$}{(First-order) Marcum \textit{Q}-function, $\alpha,\beta\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{{\small $\displaystyle Q_M(\alpha,\beta)=\frac{\int_\beta^\infty x^M e^{-\frac{x^2+{\alpha}^2}{2}}I_{M-1}(\alpha x)dx}{\alpha^{M-1}}$}}{Generalized Marcum \textit{Q}-function, $\alpha,\beta\in\mathds{R}_{0}^{+}$ and $M\in\mathds{R}^{+}$, with $Q_M(0,\beta)=\Gamma\left(M,\beta^2/2\right)/\Gamma(M)$ its limiting value for $\alpha\rightarrow0$}%
%\nomenclaturesortright{F}{{\small $Q_{M,N}(\alpha,\beta)=\int_\beta^\infty x^M e^{-\frac{x^2+\alpha^2}{2}}I_N(\alpha x)dx$}}{(Standard) Nuttall \textit{Q}-function, $\alpha,N+1\in\mathds{R}^{+}$ and $\beta,M\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{$\displaystyle \mathcal{Q}_{M,N}(\alpha,\beta)\triangleq\frac{Q_{M,N}(\alpha,\beta)}{\alpha^N}$}{Normalized Nuttall \textit{Q}-function, $\alpha,N+1\in\mathds{R}^{+}$ and $\beta,M\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{$\erfc(z)=(2/\sqrt\pi)\int_z^\infty e^{-t^2}dt$}{Complementary error function, $z\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{$Q(z)=(1/\sqrt{2\pi})\int_z^\infty e^{-t^2/2}dt$}{Gaussian \textit{Q}-function, $z\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{$\Gamma(z)=\int_0^\infty t^{z-1}e^{-t}dt$}{Euler gamma function, $z\in\mathds{R}^+$}%
%\nomenclaturesortright{F}{$\gamma\left(z,x\right)=\int_0^x t^{z-1}e^{-t}dt$}{Lower incomplete gamma function, $z\in\mathds{R}^+$, $x\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{$P(z,x)=\frac{\gamma(z,x)}{\Gamma(z)}$}{Regularized lower incomplete gamma function, $z\in\mathds{R}^+,\,x\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{$\Gamma\left(z,x\right)=\Gamma(z)-\gamma\left(z,x\right)$}{Upper incomplete gamma function, $z\in\mathds{R}^+$, $x\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{$Q(z,x)=1-P(z,x)$}{Regularized upper incomplete gamma function, ${z\in\mathds{R}^+,\,x\in\mathds{R}_{0}^{+}}$}%
%\nomenclaturesortright{F}{$\boxed{\mathcal{G}_s(z,x)\triangleq\frac{\Gamma(z+s,x)}{\Gamma(z)}}$}{Generalized incomplete gamma ratio, $z\in\mathds{R}^+$ and $s,x\in\mathds{R}_{0}^{+}$}%
%\nomenclaturesortright{F}{$\floor{x}{}$}{Integer floor function, $x\in\mathds{R}$ (maps $x$ to the largest integer less than or equal to $x$)}%
%\nomenclaturesortright{F}{$\ceil{x}{}$}{Integer ceiling function, $x\in\mathds{R}$ (maps $x$ to the smallest integer greater than or equal to $x$)}%
%\nomenclaturesortright{F}{$\boxed{\floor{x}{0.5}\triangleq\floor{x-0.5}{}+0.5}$}{Half-integer floor function, $x\in\mathds{R}$ (maps $x$ to the largest half-integer less than or equal to $x$)}%
%\nomenclaturesortright{F}{$\boxed{\ceil{x}{0.5}\triangleq\ceil{x+0.5}{}-0.5}$}{Half-integer ceiling function, $x\in\mathds{R}$ (maps $x$ to the smallest half-integer greater than or equal to $x$)}%
%\nomenclaturesortright{F}{$\boxed{\nearest{x}{0.5}\triangleq\floor{x}{}+0.5}$}{Nearest half-integer function, $x\in\mathds{R}$ (maps $x$ to its nearest half-integer)}%
%
%\nomenclaturesortright{H}{$A^c=S\setminus A$}{Complement of the set $A$ with respect to the universe $S$}%
%\nomenclaturesortright{H}{$A=\{k^2+1\colon k\in\mathds{N};k\leq 3\}$}{Set notation example for the collection $\{2,5,10\}$}%
%\nomenclaturesortright{H}{$\card{A}$}{Cardinality of the set $A$}%
%\nomenclaturesortright{H}{$\mathbb{P}(A)$}{Powerset of the set $A$}%
%\nomenclaturesortright{H}{$\boxed{S_\dag}$}{Lambda set associated with the Lambda operators}%
%\nomenclaturesortright{H}{$\boxed{N_\dag}$}{$\dag$-set associated with the canonical designs}%
%\nomenclaturesortright{H}{$\mathds{K}$}{Field such as $\mathds{C}$ or $\mathds{R}$ (general notation)}%
%\nomenclaturesortright{H}{$\mathds{C}$, $\mathds{R}$, $\mathds{Z}$}{Sets of complex, real, and integer numbers}%
%\nomenclaturesortright{H}{$\mathds{R}^{+}$, $\mathds{R}_{0}^{+}$}{Sets of positive real and non-negative real numbers}%
%\nomenclaturesortright{H}{$\mathds{N}$, $\mathds{N}_0$}{Sets of natural and non-negative integer numbers}%
%\nomenclaturesortright{H}{$\mathds{Z}+\frac{1}{2}$, $\mathds{N}_0+\frac{1}{2}$,}{Sets of half-integers and positive half-integers}%
%\nomenclaturesortright{H}{$\langle n\rangle\triangleq\{k\colon k\in\mathds{N};k\leq n\}$}{The set $\{1,\dotsc,n\}$ (shorthand notation)}%
%\nomenclaturesortright{H}{$\boxed{\{a_k\}_{k=1}^{n}}$}{The set $\{a_1,\dotsc,a_n\}$ (shorthand notation)}%
%\nomenclaturesortright{H}{$\emptyset$}{The empty set}%
%\nomenclaturesortright{H}{$\chi_{A}(x)$}{Characteristic function (a.k.a. indicator function) of the set $A$}%
%\nomenclaturesortright{H}{$\subseteq$, $\cup$, $\cap$}{Subset, union, and intersection of sets}%
%\nomenclaturesortright{H}{$\dot\vee$}{Exclusive disjunction}%
%
%\nomenclaturesortright{M}{$\mathds{C}^m$}{$m$-dimensional vector space over $\mathds{C}$ ($m\times 1$ complex vector set)}%
%\nomenclaturesortright{M}{$\mathds{C}^{m\times n}$}{$mn$-dimensional vector space over $\mathds{C}$ ($m\times n$ complex matrix~set)}%
%\nomenclaturesortright{M}{$\boldn{0}_{m}$, $\boldn{0}_{m\times n}$}{$m\times 1$ vector and $m\times n$ matrix with zero entries}%
%\nomenclaturesortright{M}{$\boldn{1}_{m}$, $\boldn{1}_{m\times n}$}{$m\times 1$ vector and $m\times n$ matrix with unit entries}%
%\nomenclaturesortright{M}{$\boldn{I}_{m}$}{Identity matrix of order $m$ (preferred over the notation $\boldn{I}_{m\times m}$ without ambiguity, since an identity matrix is always square)}%
%\nomenclaturesortright{M}{$\boldn{Z}\in\mathds{C}^{m\times n}$ with $\boldn{Z}=(z_{i,j})$}{Matrix with $(i,j)$th element $z_{i,j}\in\mathds{C}$, where $i=1:m$, $j=1:n$}%
%\nomenclaturesortright{M}{$\boldn{Z}=(\boldn{Z}_{i,j})\in\mathds{C}^{mp\times nq}$, $\boldn{Z}_{i,j}\in\mathds{C}^{p\times q}$}{Block matrix with $(i,j)$th submatrix $\boldn{Z}_{i,j}$, $i=1:m$, $j=1:n$, where $\boldn{Z}_{i,j}=(z_{\kappa,\lambda})_{i,j}$ with $\kappa=1:p$, $\lambda=1:q$}%
%\nomenclaturesortright{M}{$\boldn{Z}=(\boldn{Z}_i)\in\mathds{C}^{mp\times q}$, $\boldn{Z}_i\in\mathds{C}^{p\times q}$}{Block column vector with $i$th submatrix $\boldn{Z}_i$, $i=1:m$, where $\boldn{Z}_i=(z_{\kappa,\lambda})_i$ with $\kappa=1:p$, $\lambda=1:q$}%
%\nomenclaturesortright{M}{$\boldn{Z}=(\boldn{Z}_j)\in\mathds{C}^{p\times nq}$, $\boldn{Z}_j\in\mathds{C}^{p\times q}$}{Block row vector with $j$th submatrix $\boldn{Z}_j$, $j=1:n$, where $\boldn{Z}_j=(z_{\kappa,\lambda})_j$ with $\kappa=1:p$, $\lambda=1:q$}%
%\nomenclaturesortright{M}{$\boldn{Z}=(\boldi{z}_j)\in\mathds{C}^{m\times n}$, $\boldi{z}_j\in\mathds{C}^{m}$}{Block notation for matrix $\boldn{Z}$, partitioned into the column vectors $\boldi{z}_j$, $j=1:n$, where $\boldi{z}_j=(z_\kappa)_j$ with $\kappa=1:m$}%
%\nomenclaturesortright{M}{$\boldn{Z}=(\boldi{z}_i)\in\mathds{C}^{m\times n}$, $\boldi{z}_i\in\mathds{C}^{1\times n}$}{Block notation for matrix $\boldn{Z}$, partitioned into the row vectors $\boldi{z}_i$, $i=1:m$, where $\boldi{z}_i=(z_\kappa)_i$ with $\kappa=1:n$}%
%\nomenclaturesortright{M}{$\boldn{Z}_{m\times n}$}{Matrix $\boldn{Z}$ with $m$ rows and $n$ columns (alternative notation used to resolve any ambiguity about the size of a matrix)}%
%\nomenclaturesortright{M}{$\boldi{z}=[z_1\cdots z_n]$}{Row vector in $\mathds{C}^{1\times n}$ (brackets are used to delimit row vectors only in inline equations; parentheses delimit displayed matrices)}%
%\nomenclaturesortright{M}{$GL(n,\mathds{K})$}{Group of $n\times n$ invertible matrices over $\mathds{K}$ (general linear group)}%
%\nomenclaturesortright{M}{$\boxed{SI(n,\mathds{C})}$}{Set of $n\times n$ simple invertible matrices over $\mathds{C}$}%
%\nomenclaturesortright{M}{$D(n,\mathds{K})$}{Group of $n\times n$ nonsingular diagonal matrices over $\mathds{K}$}%
%\nomenclaturesortright{M}{$O(n,\mathds{K})$}{Group of $n\times n$ orthogonal matrices over $\mathds{K}$}%
%\nomenclaturesortright{M}{$U(n)$}{Group of $n\times n$ unitary matrices (note that $U(n)\neq O(n,\mathds{C})$)}%
%\nomenclaturesortright{M}{$P(n)$}{Group of $n\times n$ permutation matrices (\acsp{PM})}%
%\nomenclaturesortright{M}{$\boxed{\mathscr{P}_{n}}$}{Class of $n\times n$ partial \acsp{PM} of rank less or equal to $n$}%
%\nomenclaturesortright{M}{$\boxed{\mathscr{S}_{m\times n}}$}{Class of $m\times n$ sub-\acsp{PM} of rank less or equal to $\min\{m,n\}$}%
%\nomenclaturesortright{M}{$\mathscr{P}_{n}(r)$}{Set of $n\times n$ partial \acsp{PM} of rank $r$, where $0\leq r\leq n$}%
%\nomenclaturesortright{M}{$\mathscr{S}_{m\times n}(r)$}{Set of $m\times n$ sub-\acsp{PM} of rank $r$, where $0\leq r\leq\min\{m,n\}$}%
%\nomenclaturesortright{M}{$\boxed{\mathscr{G}_{m\times n}}$}{Class of $m\times n$ extended generalized \acsp{PM}}%
%\nomenclaturesortright{M}{$\re{\boldn{Z}}$, $\im{\boldn{Z}}$}{Real and imaginary parts of complex matrix $\boldn{Z}$}%
%\nomenclaturesortright{M}{${z_k}_{\kappa}$, ${z_k}_{\kappa,\lambda}$}{$\kappa$th entry of vector $\boldi{z}_k$, and $(\kappa,\lambda)$th entry of matrix $\boldn{Z}_k$}%
%\nomenclaturesortright{M}{$\boldn{I}_{(m,n)}$}{Commutation matrix of order $mn$ associated with an arbitrary $m\times n$ matrix $\boldn{A}$ according to $\vect{\boldn{A}}=\boldn{I}_{(m,n)}\vect{\boldn{A}^\intercal}$}%
%\nomenclaturesortright{M}{$\subseteq$, $+$, $\cap$}{Subspace, sum, and intersection of vector spaces}%
%\nomenclaturesortright{M}{$\dim$}{Dimension of a vector space (sometimes used in the form $\dim(\cdot)$)}%
%\nomenclaturesortright{M}{$\mathcal{C}(\boldn{Z})$, $\mathcal{C}(\boldn{Z}^\dag)$}{Column space and row space of $\boldn{Z}\in\mathds{C}^{m\times n}$ ($\dim\mathcal{C}(\boldn{Z})=\rank{\boldn{Z}}$)}%
%\nomenclaturesortright{M}{$\rank{\boldn{Z}}$}{Rank of matrix $\boldn{Z}\in\mathds{C}^{m\times n}$, $0\leq\rank{\boldn{Z}}\leq\min(m,n)$}%
%\nomenclaturesortright{M}{$\Gram{\boldi{z}_1,\dotsc,\boldi{z}_n}=(\langle\boldi{z}_j,\boldi{z}_i\rangle)\in\mathds{C}^{n\times n}$}{Gramian (or Gram) matrix of the $n$-set $\{\boldi{z}_1,\dotsc,\boldi{z}_n\}$, $\boldi{z}_j\in\mathds{C}^m$ with $i=1:n$, $j=1:n$ (equal to $\boldn{Z}^\dag\boldn{Z}$ where ${\boldn{Z}=(\boldi{z}_j)\in\mathds{C}^{m\times n}}$)}%
%\nomenclaturesortright{M}{$\boxed{\Gram{\boldi{z}}\triangleq\Gram{z_1,\dotsc,z_n}\in\mathds{C}^{n\times n}}$}{Gramian of row vector $\boldi{z}=(z_j)\in\mathds{C}^{1\times n}$ or scalar $n$-set $\{z_1,\dotsc,z_n\}$ (equal to $\boldi{z}^{\dag}\boldi{z}=(z_i^\ast z_j)$ with $i=1:n$, $j=1:n$)}%
%
%\nomenclaturesortright{O}{$x(t)\star y(t)=\int_{-\infty}^{\infty}y(\tau)x(t-\tau)d\tau$}{Convolution integral of continuous-time signals $x(t),y(t)$}%
%\nomenclaturesortright{O}{$\boldn{Z}\otimes\boldn{W}=(z_{i,j}\boldn{W})\in\mathds{C}^{mk\times nl}$}{Kronecker product of $\boldn{Z}\in\mathds{C}^{m\times n}$, $\boldn{W}\in\mathds{C}^{k\times l}$}%
%\nomenclaturesortright{O}{$\boldn{Z}\odot\boldn{W}=(\boldi{z}_j\otimes\boldi{w}_j)\in\mathds{C}^{mk\times n}$}{Column-wise Khatri-Rao product of $\boldn{Z}\in\mathds{C}^{m\times n}$, $\boldn{W}\in\mathds{C}^{k\times n}$}%
%\nomenclaturesortright{O}{$\boxed{\LambdaR{S}{\boldn{Z}}$, $\LambdaC{S}{\boldn{Z}}$, $\LambdaD{S}{\boldn{Z}}}$}{Type-$\mathcal{R}$, type-$\mathcal{C}$ and Type-$\mathcal{D}$ Lambda operators on matrix $\boldn{Z}$}%
%\nomenclaturesortright{O}{$\boxed{\LambdaRb{S}{\boldn{Z}}$, $\LambdaCb{S}{\boldn{Z}}$, $\LambdaDb{S}{\boldn{Z}}}$}{Type-$\mathcal{R}$, type-$\mathcal{C}$ and type-$\mathcal{D}$ Lambda operators on block matrix~$\boldn{Z}$}%
%\nomenclaturesortright{O}{$\biguplus\nolimits_{i\in I}A_i$}{Disjoint union of sets $A_i$, $i\in I$ ($A_i$ are pair-wise disjoint $\forall\,i$)}%
%\nomenclaturesortright{O}{$\bigoplus\nolimits_{k=1}^{m}\boldn{Z}_k\triangleq\boldn{Z}_1\oplus\boldn{Z}_2\oplus\dotsm\oplus\boldn{Z}_m$}{Direct sum of $\boldn{Z}_k\in\mathds{C}^{p\times q}$, $k=1:m$, also written as $\diag{\boldn{Z}_k}_m$ (it is also used for the sum of disjoint vector subspaces)}%
%\nomenclaturesortright{O}{$\boldn{Z}\circ\boldn{W}=(z_{i,j}w_{i,j})\in\mathds{C}^{m\times n}$}{Hadamard product (a.k.a. Schur product) of $\boldn{Z},\boldn{W}\in\mathds{C}^{m\times n}$}%
%\nomenclaturesortright{O}{$\vect{\boldn{Z}}\colon\mathds{C}^{m\times n}\to\mathds{C}^{mn}$}{Vectorization of matrix $\boldn{Z}\in\mathds{C}^{m\times n}$ (by stacking its columns)}%
%\nomenclaturesortright{O}{$\norm{\boldn{Z}}_{F}=(\sum_{i=1}^{m}\sum_{j=1}^{n}\abs{z_{i,j}}^2)^{1/2}$}{Frobenius norm of matrix $\boldn{Z}\in\mathds{C}^{m\times n}$}%
%\nomenclaturesortright{O}{$\trace{\boldn{Z}}=\sum_{i=1}^{m}z_{i,i}$}{Trace of complex square matrix $\boldn{Z}$ of order $m$}%
%\nomenclaturesortright{O}{$\boxed{\diag{\boldn{Z}_k}_m\triangleq\diag{\boldn{Z}_1,\dotsc,\boldn{Z}_m}}$}{Block diagonal matrix with $\boldn{Z}_k$, $k=1:m$, in main diagonal}%
%\nomenclaturesortright{O}{$\boxed{\diag{z_k}_m\triangleq\diag{z_1,\dotsc,z_m}}$}{Diagonal matrix with $z_k$, $k=1:m$, in main diagonal}%
%\nomenclaturesortright{O}{$\boldn{Z}^\dag=(\boldn{Z}^\intercal)^\ast=(\boldn{Z}^\ast)^\intercal$}{Hermitian (or conjugate) transpose of complex matrix $\boldn{Z}$}%
%\nomenclaturesortright{O}{$\boldn{Z}^\intercal$, $\boldn{Z}^\ast$}{Transpose and complex conjugate of complex matrix $\boldn{Z}$}%
%\nomenclaturesortright{O}{$\det(\boldn{Z})$}{Determinant of complex square matrix $\boldn{Z}$}%
%\nomenclaturesortright{O}{$\boldn{Z}^{-1}$}{Inverse of complex (square) nonsingular matrix $\boldn{Z}$}%
%\nomenclaturesortright{O}{$\boldn{Z}^-$ with $\boldn{Z}\boldn{Z}^-\boldn{Z}=\boldn{Z}$}{Generalized (or weak) inverse of arbitrary complex matrix $\boldn{Z}$}%
%\nomenclaturesortright{O}{$\boldn{Z}^+=(\boldn{Z}^\dag\boldn{Z})^{-1}\boldn{Z}^\dag$ with $\boldn{Z}^+\boldn{Z}=\boldn{I}_n$}{Moore-Penrose inverse of $\boldn{Z}\in\mathds{C}^{m\times n}$ with full column rank}%
%\nomenclaturesortright{O}{$\norm{\boldi{z}}_p=(\sum_{i=1}^{m}\abs{z_i}^p)^{1/p}$}{$L_p$ norm of vector $\boldi{z}\in\mathds{C}^{m}$ with $p-1\in\mathds{R}_{0}^{+}$ ($\norm{\boldi{z}}_2=\norm{\boldi{z}}$)}%
%\nomenclaturesortright{O}{$\norm{\boldi{z}}=(\sum_{i=1}^{m}\abs{z_i}^2)^{1/2}$}{Euclidean norm (a.k.a. length) of vector $\boldi{z}\in\mathds{C}^{m}$}%
%\nomenclaturesortright{O}{$\langle\boldi{z},\boldi{w}\rangle=\boldi{z}^\intercal\boldi{w}^\ast=\boldi{w}^\dag\boldi{z}$}{Hermitian inner (or dot) product of $\boldi{z},\boldi{w}\in\mathds{C}^{m}$ ($\langle\boldi{z},\boldi{z}\rangle=\norm{\boldi{z}}^2$)}%
%
%\nomenclaturesortright{R}{$\var{z}=\av{\abs{z-\mu_{z}}^2}$}{Variance of \acs{RV} $z\in\mathds{C}$}%
%\nomenclaturesortright{R}{$\sigma_z=\sqrt{\var{z}}$}{Standard deviation of \acs{RV} $z\in\mathds{C}$}%
%\nomenclaturesortright{R}{$\cov{z,w}=\av{(z-\mu_{z})(w-\mu_{w})^\ast}$}{Covariance of \acsp{RV} $z,w\in\mathds{C}$}%
%\nomenclaturesortright{R}{$\mathrm{K}_\boldn{Z}=\av{(\boldn{Z}-\mu_{\boldn{Z}})(\boldn{Z}-\mu_{\boldn{Z}})^\dag}$}{Covariance matrix of random $\boldn{Z}\in\mathds{C}^{m\times n}$}%
%\nomenclaturesortright{R}{$\mathrm{M}_\boldn{Z}=\av{(\boldn{Z}-\mu_{\boldn{Z}})(\boldn{Z}-\mu_{\boldn{Z}})^\intercal}$}{Pseudo-covariance (or correlation) matrix of random $\boldn{Z}\in\mathds{C}^{m\times n}$}%
%\nomenclaturesortright{R}{$f_{x}(y)$, $F_{x}(y)$}{\acs{PDF} and \acs{CDF} of (generally complex) \acs{RV} $x$ evaluated at $x=y$}%
%\nomenclaturesortright{R}{$\mu_x=\av{x}=\int_{-\infty}^{\infty}xf_{x}(x)dx$}{Expected value (or mean) of \acs{RV} $x\in\mathds{R}$}%
%\nomenclaturesortright{R}{$\mu_\boldn{Z}=\av{\boldn{Z}}$}{Mean of random $\boldn{Z}\in\mathds{C}^{m\times n}$}%
%
%\nomenclaturesortright{S}{$\mathcal{S}_{x}(f)=\ft{\tau}{\mathcal{R}_{x}(\tau)}$}{\acs{PSD} of a \acs{WSS} stochastic process $\{x(t)\}$ (Wiener-Khinchin Th.)}%
%\nomenclaturesortright{S}{$\mathcal{R}_{z}(t+\tau,t)=\av{z(t+\tau)z^\ast(t)}$}{Autocorrelation function of complex random signal $z(t)$}%
%\nomenclaturesortright{S}{$\mathcal{P}_{x}=\underset{T\rightarrow\infty}{\lim}\frac{1}{2T}\int_{-T}^{T}\abs{x(t)}^2dt$}{(Time) average power of stochastic process $\{x(t)\}$}%
%\nomenclaturesortright{S}{$\mathcal{R}_{zw}(t+\tau,t)=\av{z(t+\tau)w^\ast(t)}$}{Cross-correlation function of complex random signals $z(t),w(t)$}%
%\nomenclaturesortright{S}{$\mu_{x}(t)=\av{x(t)}$}{Mean function of real random signal $x(t)$}%
%
%\nomenclaturesortright{T}{$\ft{t}{x(t)}=\int_{-\infty}^{\infty}x(t)e^{-\jmath2\pi ft}dt$}{Fourier transform of function $x(t)$ with respect to $t$}%
%\nomenclaturesortright{T}{$\ift{f}{X(f)}=\int_{-\infty}^{\infty}X(f)e^{\jmath2\pi ft}df$}{Inverse Fourier transform of function $X(f)$ with respect to $f$}%
%\nomenclaturesortright{T}{$T\colon X\to Y$}{Mapping rule (e.g., transformation, operator, function) from $X$ to $Y$ such that $\forall\,x\in X$ there is a unique object $T(x)\in Y$}%
%\nomenclaturesortright{T}{$x\mapsto T(x)$}{Mapping from $x$ to $T(x)$, also defining the mapping rule $T$}%
%
%\nomenclaturesortright{Z}{$k=m:n$}{Values of $k$ equal to $m,m+1,\dotsc,n$ with $k,m,n\in\mathds{N}$, $n>m$}%
%\nomenclaturesortright{Z}{$x=a:c:b$}{Values of $x$ equal to $a,a+c,\dotsc,b$ with $x,a,b,c\in\mathds{R}$, $\frac{b-a}{c}\in\mathds{N}$}%
%\nomenclaturesortright{Z}{$\delta_{ij}$}{Kronecker delta with $\delta_{ij}=1$ for $i=j$; $=0$ for $i\neq j$}%
%\nomenclaturesortright{Z}{$z$, $\boldi{z}$, $\boldn{Z}$}{Scalar in $\mathds{K}$, vector in $\mathds{K}^{m}$ or $\mathds{K}^{1\times m}$, and matrix in $\mathds{K}^{m\times n}$}%
%\nomenclaturesortright{Z}{$\forall$, $\exists$, $\in$, $\notin$, $\Rightarrow$}{For each, there exists, member of, not a member of, implies}%
%\nomenclaturesortright{Z}{$\equiv$}{Equivalence (not to be confused with the equivalence relation)}%
%\nomenclaturesortright{Z}{$\defeq$}{Assignment in the sense of $\leftarrow$ (i.e., takes the value of)}%
%\nomenclaturesortright{Z}{$\defeqr$}{Assignment in the sense of $\rightarrow$ (i.e., gives its value to)}%
%\nomenclaturesortright{Z}{$\sim$}{Equivalence relation (used also between \acsp{RV} and \acsp{PDF})}%
%\nomenclaturesortright{Z}{$\triangleq$}{Equality by definition}%
%\nomenclaturesortright{Z}{$\prod_{k=1}^n a_k$}{Product $a_1a_2\dotsm a_n$ (not to be confused with the $\Pi(\cdot)$ function)}%
%\nomenclaturesortright{Z}{$(a_k)_{k=1}^{n}=(a_1,\dotsc,a_n)$}{Finite sequence of length $n$ or $n$-tuple (shorthand notation)}%
%\nomenclaturesortright{Z}{$(x,y)$}{Ordered pair or $2$-tuple (not to be confused with the set $\{x,y\}$)}%
%\nomenclaturesortright{Z}{$\times$}{Multiplication sign (used to indicate the size of matrices and \acs{MIMO} arrays, and to emphasize the product of two quantities)}%
%\nomenclaturesortright{Z}{$\bullet$, $\divideontimes$}{Nonzero entry of a matrix, and unary/binary operator}%
%\nomenclaturesortright{Z}{$\frac{\partial}{\partial{v}}$}{Partial derivative with respect to $v$}%
%\nomenclaturesortright{Z}{$\delta_x=x-\floor{x}{}$}{Fractional part of $x\in\mathds{R}_{0}^{+}$ with $\delta_x\in [0,1)$}%
%\nomenclaturesortright{Z}{iff}{If and only if}%
%\else\fi
%
%%Symbols and notations for chapter 3
%\ifchapterthreeflag
%\else\fi
%
%%Symbols and notations for chapter 4
%\ifchapterfourflag
%\else\fi
%
%%Symbols and notations for chapter 5
%\ifchapterfiveflag
%\else\fi

